Parameter and density estimation from real-world traffic data: A kinetic compartmental approach

The main motivation of this work is to assess the validity of a LWR traffic flow model to model measurements obtained from trajectory data, and propose extensions of this model to improve it. A formulation for a discrete dynamical system is proposed aiming at reproducing the evolution in time of the density of vehicles along a road, as observed in the measurements. This system is formulated as a chemical reaction network where road cells are interpreted as compartments, the transfer of vehicles from one cell to the other is seen as a chemical reaction between adjacent compartment and the density of vehicles is seen as a concentration of reactant. Several degrees of flexibility on the parameters of this system, which basically consist of the reaction rates between the compartments, can be considered: a constant value or a function depending on time and/or space. Density measurements coming from trajectory data are then interpreted as observations of the states of this system at consecutive times. Optimal reaction rates for the system are then obtained by minimizing the discrepancy between the output of the system and the state measurements. This approach was tested both on simulated and real data, proved successful in recreating the complexity of traffic flows despite the assumptions on the flux-density relation.

==> fig/lxf_1_param0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.9943867743175702, 0.7938485198000773, 0.4740484429065747}{\scriptsize{ 0.64}} &   \cellcolor[rgb]{0.796078431372549, 0.9135717031910804, 0.5095732410611303}{\scriptsize{ 0.37}} & \cellcolor[rgb]{0.27143406382160706, 0.6785851595540177, 0.35609381007304886}{\scriptsize{ 0.16}} & \cellcolor[rgb]{0.15455594002306805, 0.621683967704729, 0.32687427912341405}{\scriptsize{ 0.12}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.9948481353325644, 0.8169165705497887, 0.4934256055363323}{\scriptsize{ 0.63}} & \cellcolor[rgb]{0.7411764705882352, 0.8898885044213763, 0.47404844290657433}{\scriptsize{ 0.34}} & \cellcolor[rgb]{0.21299500192233758, 0.6501345636293733, 0.34148404459823145}{\scriptsize{ 0.14}} & \cellcolor[rgb]{0.14286812764321416, 0.6159938485198001, 0.3239523260284506}{\scriptsize{ 0.11}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.9956170703575548, 0.8553633217993082, 0.5257208765859286}{\scriptsize{ 0.61}} &  \cellcolor[rgb]{0.7568627450980391, 0.8966551326412917, 0.4841983852364474}{\scriptsize{ 0.35}} &   \cellcolor[rgb]{0.17793156478277586, 0.6330642060745867, 0.332718185313341}{\scriptsize{ 0.13}} & \cellcolor[rgb]{0.14286812764321416, 0.6159938485198001, 0.3239523260284506}{\scriptsize{ 0.11}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.40984236831987697, 0.7454825067281815, 0.3893118031526336}{\scriptsize{ 0.20}} &  \cellcolor[rgb]{0.8196078431372548, 0.9237216455209534, 0.5247981545559399}{\scriptsize{ 0.39}} & \cellcolor[rgb]{0.25974625144175323, 0.6728950403690889, 0.35317185697808534}{\scriptsize{ 0.15}} & \cellcolor[rgb]{0.14286812764321416, 0.6159938485198001, 0.3239523260284506}{\scriptsize{ 0.11}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.9734717416378317, 0.5474048442906576, 0.3181084198385237}{\scriptsize{ 0.75}} &  \cellcolor[rgb]{0.8568242983467896, 0.9397154940407536, 0.5530949634755863}{\scriptsize{ 0.41}} &   \cellcolor[rgb]{0.1896193771626297, 0.6387543252595156, 0.3356401384083045}{\scriptsize{ 0.13}} & \cellcolor[rgb]{0.14286812764321416, 0.6159938485198001, 0.3239523260284506}{\scriptsize{ 0.12}} \\
\bottomrule
\end{tabular}


==> fig/lxf_1_param1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.7470203767781622, 0.09596309111880047, 0.15101883890811227}{\scriptsize{ 0.95}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                 \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6547481737793157, 0.007381776239907711, 0.14917339484813533}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.8453671664744329, 0.19292579777008845, 0.15509419454056134}{\scriptsize{ 0.90}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                 \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.6624375240292195, 0.014763552479815478, 0.1493271818531334}{\scriptsize{ 0.99}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.8085351787773933, 0.15501730103806227, 0.1522491349480969}{\scriptsize{ 0.91}} &  \cellcolor[rgb]{0.6624375240292195, 0.014763552479815478, 0.1493271818531334}{\scriptsize{ 0.99}} & \cellcolor[rgb]{0.6547481737793157, 0.007381776239907711, 0.14917339484813533}{\scriptsize{ 1.00}} \\
\bottomrule
\end{tabular}


==> fig/lxf_1_rmse0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
 \cellcolor[rgb]{0.12087658592848904, 0.4956862745098039, 0.7186159169550173}{\scriptsize{ 0.220}} &  \cellcolor[rgb]{0.14196078431372547, 0.5976470588235294, 0.756078431372549}{\scriptsize{ 0.157}} & \cellcolor[rgb]{0.17739331026528254, 0.6340638216070742, 0.7600153787004998}{\scriptsize{ 0.137}} & \cellcolor[rgb]{0.22611303344867356, 0.6841368704344483, 0.7654286812764322}{\scriptsize{ 0.113}} & \cellcolor[rgb]{0.27397154940407537, 0.7207996924259901, 0.7658592848904268}{\scriptsize{ 0.096}} \\
 \cellcolor[rgb]{0.12149173394848135, 0.4894117647058823, 0.7156632064590542}{\scriptsize{ 0.222}} &  \cellcolor[rgb]{0.14196078431372547, 0.5976470588235294, 0.756078431372549}{\scriptsize{ 0.159}} & \cellcolor[rgb]{0.17739331026528254, 0.6340638216070742, 0.7600153787004998}{\scriptsize{ 0.138}} &   \cellcolor[rgb]{0.2305420991926182, 0.6886889657823914, 0.765920799692426}{\scriptsize{ 0.111}} &    \cellcolor[rgb]{0.28159938485198, 0.7236293733179546, 0.7647520184544406}{\scriptsize{ 0.094}} \\
 \cellcolor[rgb]{0.12210688196847366, 0.4831372549019608, 0.7127104959630911}{\scriptsize{ 0.227}} &  \cellcolor[rgb]{0.1463898500576701, 0.6021991541714725, 0.7565705497885429}{\scriptsize{ 0.157}} & \cellcolor[rgb]{0.18182237600922718, 0.6386159169550173, 0.7605074971164937}{\scriptsize{ 0.135}} &   \cellcolor[rgb]{0.2305420991926182, 0.6886889657823914, 0.765920799692426}{\scriptsize{ 0.110}} &    \cellcolor[rgb]{0.28159938485198, 0.7236293733179546, 0.7647520184544406}{\scriptsize{ 0.094}} \\
 \cellcolor[rgb]{0.12333717800845828, 0.47058823529411764, 0.706805074971165}{\scriptsize{ 0.233}} & \cellcolor[rgb]{0.11538638985005764, 0.5703344867358708, 0.7531257208765859}{\scriptsize{ 0.175}} &  \cellcolor[rgb]{0.16853517877739327, 0.624959630911188, 0.7590311418685122}{\scriptsize{ 0.143}} & \cellcolor[rgb]{0.21725490196078429, 0.6750326797385621, 0.7644444444444445}{\scriptsize{ 0.116}} &  \cellcolor[rgb]{0.26634371395617074, 0.7179700115340254, 0.766966551326413}{\scriptsize{ 0.098}} \\
\cellcolor[rgb]{0.12395232602845059, 0.46431372549019606, 0.7038523644752018}{\scriptsize{ 0.238}} & \cellcolor[rgb]{0.12867358708189156, 0.5839907727797001, 0.7546020761245674}{\scriptsize{ 0.166}} &  \cellcolor[rgb]{0.16853517877739327, 0.624959630911188, 0.7590311418685122}{\scriptsize{ 0.141}} & \cellcolor[rgb]{0.23497116493656298, 0.6932410611303347, 0.7664129181084199}{\scriptsize{ 0.109}} &  \cellcolor[rgb]{0.2526874279123414, 0.7114494425221068, 0.7683813917723953}{\scriptsize{ 0.101}} \\
\bottomrule
\end{tabular}


==> fig/lxf_1_rmse1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
 \cellcolor[rgb]{0.12087658592848904, 0.4956862745098039, 0.7186159169550173}{\scriptsize{ 0.220}} &  \cellcolor[rgb]{0.14196078431372547, 0.5976470588235294, 0.756078431372549}{\scriptsize{ 0.157}} & \cellcolor[rgb]{0.17739331026528254, 0.6340638216070742, 0.7600153787004998}{\scriptsize{ 0.138}} &  \cellcolor[rgb]{0.21282583621683965, 0.670480584390619, 0.7639523260284506}{\scriptsize{ 0.118}} & \cellcolor[rgb]{0.23940023068050748, 0.6977931564782776, 0.7669050365244138}{\scriptsize{ 0.106}} \\
 \cellcolor[rgb]{0.12149173394848135, 0.4894117647058823, 0.7156632064590542}{\scriptsize{ 0.222}} &  \cellcolor[rgb]{0.14196078431372547, 0.5976470588235294, 0.756078431372549}{\scriptsize{ 0.159}} &   \cellcolor[rgb]{0.1729642445213379, 0.6295117262591311, 0.759523260284506}{\scriptsize{ 0.139}} & \cellcolor[rgb]{0.21725490196078429, 0.6750326797385621, 0.7644444444444445}{\scriptsize{ 0.116}} & \cellcolor[rgb]{0.24825836216839675, 0.7068973471741637, 0.7678892733564014}{\scriptsize{ 0.103}} \\
 \cellcolor[rgb]{0.12210688196847366, 0.4831372549019608, 0.7127104959630911}{\scriptsize{ 0.227}} &  \cellcolor[rgb]{0.14196078431372547, 0.5976470588235294, 0.756078431372549}{\scriptsize{ 0.157}} & \cellcolor[rgb]{0.18182237600922718, 0.6386159169550173, 0.7605074971164937}{\scriptsize{ 0.136}} & \cellcolor[rgb]{0.22168396770472892, 0.6795847750865052, 0.7649365628604383}{\scriptsize{ 0.115}} & \cellcolor[rgb]{0.24825836216839675, 0.7068973471741637, 0.7678892733564014}{\scriptsize{ 0.103}} \\
 \cellcolor[rgb]{0.12333717800845828, 0.47058823529411764, 0.706805074971165}{\scriptsize{ 0.233}} & \cellcolor[rgb]{0.11538638985005764, 0.5703344867358708, 0.7531257208765859}{\scriptsize{ 0.175}} &  \cellcolor[rgb]{0.16410611303344877, 0.620407535563245, 0.7585390234525183}{\scriptsize{ 0.144}} &  \cellcolor[rgb]{0.21282583621683965, 0.670480584390619, 0.7639523260284506}{\scriptsize{ 0.119}} &  \cellcolor[rgb]{0.2438292964244521, 0.7023452518262207, 0.7673971549404076}{\scriptsize{ 0.105}} \\
\cellcolor[rgb]{0.12395232602845059, 0.46431372549019606, 0.7038523644752018}{\scriptsize{ 0.238}} & \cellcolor[rgb]{0.12867358708189156, 0.5839907727797001, 0.7546020761245674}{\scriptsize{ 0.166}} &  \cellcolor[rgb]{0.16853517877739327, 0.624959630911188, 0.7590311418685122}{\scriptsize{ 0.142}} & \cellcolor[rgb]{0.22168396770472892, 0.6795847750865052, 0.7649365628604383}{\scriptsize{ 0.114}} & \cellcolor[rgb]{0.23497116493656298, 0.6932410611303347, 0.7664129181084199}{\scriptsize{ 0.108}} \\
\bottomrule
\end{tabular}


==> fig/lxf_3_param0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.4295271049596309, 0.7540945790080739, 0.3914648212226067}{\scriptsize{ 0.21}} & \cellcolor[rgb]{0.16624375240292197, 0.6273740868896578, 0.32979623221837756}{\scriptsize{ 0.12}} & \cellcolor[rgb]{0.10780469050365243, 0.5989234909650134, 0.31518646674356016}{\scriptsize{ 0.10}} &   \cellcolor[rgb]{0.0839677047289504, 0.5628604382929643, 0.2964244521337947}{\scriptsize{ 0.09}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.4492118415993849, 0.7627066512879662, 0.39361783929257976}{\scriptsize{ 0.22}} &  \cellcolor[rgb]{0.11949250288350635, 0.6046136101499423, 0.3181084198385236}{\scriptsize{ 0.11}} &  \cellcolor[rgb]{0.09996155324875047, 0.5923875432525951, 0.3118031526336025}{\scriptsize{ 0.10}} &   \cellcolor[rgb]{0.0839677047289504, 0.5628604382929643, 0.2964244521337947}{\scriptsize{ 0.08}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.4295271049596309, 0.7540945790080739, 0.3914648212226067}{\scriptsize{ 0.21}} & \cellcolor[rgb]{0.10780469050365243, 0.5989234909650134, 0.31518646674356016}{\scriptsize{ 0.10}} &  \cellcolor[rgb]{0.09596309111880046, 0.5850057670126874, 0.3079584775086505}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.07996924259900039, 0.5554786620530565, 0.29257977700884275}{\scriptsize{ 0.08}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.7568627450980391, 0.8966551326412917, 0.4841983852364474}{\scriptsize{ 0.35}} &  \cellcolor[rgb]{0.11949250288350635, 0.6046136101499423, 0.3181084198385236}{\scriptsize{ 0.11}} &  \cellcolor[rgb]{0.09996155324875047, 0.5923875432525951, 0.3118031526336025}{\scriptsize{ 0.10}} &   \cellcolor[rgb]{0.0839677047289504, 0.5628604382929643, 0.2964244521337947}{\scriptsize{ 0.08}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.5968473663975393, 0.8272971933871587, 0.40976547481737796}{\scriptsize{ 0.28}} &  \cellcolor[rgb]{0.11949250288350635, 0.6046136101499423, 0.3181084198385236}{\scriptsize{ 0.11}} &  \cellcolor[rgb]{0.09596309111880046, 0.5850057670126874, 0.3079584775086505}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.08796616685890042, 0.5702422145328719, 0.30026912725874666}{\scriptsize{ 0.09}} \\
\bottomrule
\end{tabular}


==> fig/lxf_3_param1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                 \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                 \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6624375240292195, 0.014763552479815478, 0.1493271818531334}{\scriptsize{ 0.99}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6547481737793157, 0.007381776239907711, 0.14917339484813533}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                 \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6701268742791234, 0.02214532871972319, 0.14948096885813147}{\scriptsize{ 0.99}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} \\
\bottomrule
\end{tabular}


==> fig/lxf_3_rmse0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.11472510572856594, 0.5584313725490195, 0.7481430219146482}{\scriptsize{ 0.184}} &  \cellcolor[rgb]{0.2438292964244521, 0.7023452518262207, 0.7673971549404076}{\scriptsize{ 0.104}} &  \cellcolor[rgb]{0.3197385620915033, 0.7377777777777779, 0.7592156862745099}{\scriptsize{ 0.085}} & \cellcolor[rgb]{0.38076124567474046, 0.7604152249134948, 0.7503575547866205}{\scriptsize{ 0.075}} & \cellcolor[rgb]{0.45703960015378703, 0.7887120338331411, 0.7392848904267589}{\scriptsize{ 0.062}} \\
\cellcolor[rgb]{0.11595540176855056, 0.5458823529411765, 0.7422376009227221}{\scriptsize{ 0.191}} &  \cellcolor[rgb]{0.2438292964244521, 0.7023452518262207, 0.7673971549404076}{\scriptsize{ 0.105}} &  \cellcolor[rgb]{0.3197385620915033, 0.7377777777777779, 0.7592156862745099}{\scriptsize{ 0.086}} & \cellcolor[rgb]{0.38076124567474046, 0.7604152249134948, 0.7503575547866205}{\scriptsize{ 0.074}} & \cellcolor[rgb]{0.44941176470588234, 0.7858823529411765, 0.7403921568627451}{\scriptsize{ 0.063}} \\
\cellcolor[rgb]{0.11595540176855056, 0.5458823529411765, 0.7422376009227221}{\scriptsize{ 0.190}} & \cellcolor[rgb]{0.24825836216839675, 0.7068973471741637, 0.7678892733564014}{\scriptsize{ 0.104}} & \cellcolor[rgb]{0.30448289119569394, 0.7321184159938485, 0.7614302191464821}{\scriptsize{ 0.089}} & \cellcolor[rgb]{0.38076124567474046, 0.7604152249134948, 0.7503575547866205}{\scriptsize{ 0.074}} &  \cellcolor[rgb]{0.4417839292579777, 0.7830526720492119, 0.7414994232987312}{\scriptsize{ 0.064}} \\
 \cellcolor[rgb]{0.1190311418685121, 0.5145098039215686, 0.7274740484429065}{\scriptsize{ 0.208}} &  \cellcolor[rgb]{0.20396770472895037, 0.6613763936947328, 0.762968089196463}{\scriptsize{ 0.122}} &    \cellcolor[rgb]{0.28159938485198, 0.7236293733179546, 0.7647520184544406}{\scriptsize{ 0.094}} &  \cellcolor[rgb]{0.3502499038831219, 0.7490965013456363, 0.7547866205305652}{\scriptsize{ 0.080}} &  \cellcolor[rgb]{0.4265282583621684, 0.7773933102652826, 0.7437139561707036}{\scriptsize{ 0.067}} \\
\cellcolor[rgb]{0.12149173394848135, 0.4894117647058823, 0.7156632064590542}{\scriptsize{ 0.223}} & \cellcolor[rgb]{0.22611303344867356, 0.6841368704344483, 0.7654286812764322}{\scriptsize{ 0.113}} & \cellcolor[rgb]{0.27397154940407537, 0.7207996924259901, 0.7658592848904268}{\scriptsize{ 0.096}} & \cellcolor[rgb]{0.38076124567474046, 0.7604152249134948, 0.7503575547866205}{\scriptsize{ 0.074}} &  \cellcolor[rgb]{0.4112725874663591, 0.7717339484813533, 0.7459284890426758}{\scriptsize{ 0.069}} \\
\bottomrule
\end{tabular}


==> fig/lxf_3_rmse1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.11472510572856594, 0.5584313725490195, 0.7481430219146482}{\scriptsize{ 0.184}} & \cellcolor[rgb]{0.23497116493656298, 0.6932410611303347, 0.7664129181084199}{\scriptsize{ 0.109}} &  \cellcolor[rgb]{0.26634371395617074, 0.7179700115340254, 0.766966551326413}{\scriptsize{ 0.098}} &  \cellcolor[rgb]{0.2892272202998847, 0.7264590542099193, 0.7636447520184545}{\scriptsize{ 0.092}} &  \cellcolor[rgb]{0.3121107266435986, 0.7349480968858132, 0.760322952710496}{\scriptsize{ 0.087}} \\
\cellcolor[rgb]{0.11595540176855056, 0.5458823529411765, 0.7422376009227221}{\scriptsize{ 0.191}} &   \cellcolor[rgb]{0.2305420991926182, 0.6886889657823914, 0.765920799692426}{\scriptsize{ 0.109}} & \cellcolor[rgb]{0.27397154940407537, 0.7207996924259901, 0.7658592848904268}{\scriptsize{ 0.096}} & \cellcolor[rgb]{0.30448289119569394, 0.7321184159938485, 0.7614302191464821}{\scriptsize{ 0.089}} & \cellcolor[rgb]{0.3273663975394079, 0.7406074586697424, 0.7581084198385236}{\scriptsize{ 0.084}} \\
\cellcolor[rgb]{0.11595540176855056, 0.5458823529411765, 0.7422376009227221}{\scriptsize{ 0.190}} & \cellcolor[rgb]{0.23497116493656298, 0.6932410611303347, 0.7664129181084199}{\scriptsize{ 0.108}} &  \cellcolor[rgb]{0.26634371395617074, 0.7179700115340254, 0.766966551326413}{\scriptsize{ 0.098}} & \cellcolor[rgb]{0.30448289119569394, 0.7321184159938485, 0.7614302191464821}{\scriptsize{ 0.089}} & \cellcolor[rgb]{0.3273663975394079, 0.7406074586697424, 0.7581084198385236}{\scriptsize{ 0.084}} \\
 \cellcolor[rgb]{0.1190311418685121, 0.5145098039215686, 0.7274740484429065}{\scriptsize{ 0.208}} &  \cellcolor[rgb]{0.20396770472895037, 0.6613763936947328, 0.762968089196463}{\scriptsize{ 0.124}} &  \cellcolor[rgb]{0.2526874279123414, 0.7114494425221068, 0.7683813917723953}{\scriptsize{ 0.101}} &  \cellcolor[rgb]{0.2892272202998847, 0.7264590542099193, 0.7636447520184545}{\scriptsize{ 0.092}} & \cellcolor[rgb]{0.3273663975394079, 0.7406074586697424, 0.7581084198385236}{\scriptsize{ 0.085}} \\
\cellcolor[rgb]{0.12149173394848135, 0.4894117647058823, 0.7156632064590542}{\scriptsize{ 0.223}} & \cellcolor[rgb]{0.22168396770472892, 0.6795847750865052, 0.7649365628604383}{\scriptsize{ 0.115}} & \cellcolor[rgb]{0.24825836216839675, 0.7068973471741637, 0.7678892733564014}{\scriptsize{ 0.103}} &   \cellcolor[rgb]{0.3121107266435986, 0.7349480968858132, 0.760322952710496}{\scriptsize{ 0.088}} & \cellcolor[rgb]{0.3197385620915033, 0.7377777777777779, 0.7592156862745099}{\scriptsize{ 0.086}} \\
\bottomrule
\end{tabular}


==> fig/lxf_5_param0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.9345636293733179, 0.38054594386774315, 0.24121491733948483}{\scriptsize{ 0.82}} &   \cellcolor[rgb]{0.17793156478277586, 0.6330642060745867, 0.332718185313341}{\scriptsize{ 0.13}} & \cellcolor[rgb]{0.10780469050365243, 0.5989234909650134, 0.31518646674356016}{\scriptsize{ 0.10}} &   \cellcolor[rgb]{0.0839677047289504, 0.5628604382929643, 0.2964244521337947}{\scriptsize{ 0.08}} & \cellcolor[rgb]{0.06797385620915032, 0.5333333333333333, 0.28104575163398693}{\scriptsize{ 0.07}} \\
\cellcolor[rgb]{0.7085736255286429, 0.05905420991926183, 0.15024990388312187}{\scriptsize{ 0.97}} &   \cellcolor[rgb]{0.17793156478277586, 0.6330642060745867, 0.332718185313341}{\scriptsize{ 0.13}} &  \cellcolor[rgb]{0.09596309111880046, 0.5850057670126874, 0.3079584775086505}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.07996924259900039, 0.5554786620530565, 0.29257977700884275}{\scriptsize{ 0.08}} &  \cellcolor[rgb]{0.0639753940792003, 0.5259515570934256, 0.27720107650903497}{\scriptsize{ 0.06}} \\
\cellcolor[rgb]{0.7700884275278739, 0.11810841983852365, 0.15148019992310652}{\scriptsize{ 0.93}} & \cellcolor[rgb]{0.16624375240292197, 0.6273740868896578, 0.32979623221837756}{\scriptsize{ 0.12}} & \cellcolor[rgb]{0.09196462898885044, 0.5776239907727797, 0.30411380238369856}{\scriptsize{ 0.09}} & \cellcolor[rgb]{0.07597078046905037, 0.5480968858131487, 0.28873510188389084}{\scriptsize{ 0.08}} & \cellcolor[rgb]{0.05997693194925029, 0.5185697808535179, 0.27335640138408307}{\scriptsize{ 0.06}} \\
                \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.37662437524029213, 0.7297962322183775, 0.3823913879277201}{\scriptsize{ 0.19}} &  \cellcolor[rgb]{0.09596309111880046, 0.5850057670126874, 0.3079584775086505}{\scriptsize{ 0.09}} &   \cellcolor[rgb]{0.0839677047289504, 0.5628604382929643, 0.2964244521337947}{\scriptsize{ 0.08}} &  \cellcolor[rgb]{0.0639753940792003, 0.5259515570934256, 0.27720107650903497}{\scriptsize{ 0.06}} \\
                \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &    \cellcolor[rgb]{0.24805843906189928, 0.66720492118416, 0.3502499038831219}{\scriptsize{ 0.15}} & \cellcolor[rgb]{0.09196462898885044, 0.5776239907727797, 0.30411380238369856}{\scriptsize{ 0.09}} & \cellcolor[rgb]{0.07597078046905037, 0.5480968858131487, 0.28873510188389084}{\scriptsize{ 0.08}} & \cellcolor[rgb]{0.06797385620915032, 0.5333333333333333, 0.28104575163398693}{\scriptsize{ 0.07}} \\
\bottomrule
\end{tabular}


==> fig/lxf_5_param1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &    \cellcolor[rgb]{0.9152633602460591, 0.964321414840446, 0.6330642060745867}{\scriptsize{ 0.44}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &   \cellcolor[rgb]{0.8626682045367167, 0.9421760861207228, 0.5610918877354863}{\scriptsize{ 0.41}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6547481737793157, 0.007381776239907711, 0.14917339484813533}{\scriptsize{ 0.99}} &   \cellcolor[rgb]{0.7725490196078431, 0.9034217608612072, 0.4943483275663206}{\scriptsize{ 0.36}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &                  \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.9345636293733179, 0.38054594386774315, 0.24121491733948483}{\scriptsize{ 0.82}} \\
\cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} &  \cellcolor[rgb]{0.21299500192233758, 0.6501345636293733, 0.34148404459823145}{\scriptsize{ 0.14}} &  \cellcolor[rgb]{0.04798154555940023, 0.4964244521337947, 0.2618223760092272}{\scriptsize{ 0.05}} \\
\bottomrule
\end{tabular}


==> fig/lxf_5_rmse0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.14196078431372547, 0.5976470588235294, 0.756078431372549}{\scriptsize{ 0.157}} & \cellcolor[rgb]{0.34262206843521725, 0.7462668204536717, 0.7558938869665514}{\scriptsize{ 0.081}} &   \cellcolor[rgb]{0.4189004229142639, 0.774563629373318, 0.7448212226066897}{\scriptsize{ 0.067}} &  \cellcolor[rgb]{0.4722952710495963, 0.7943713956170704, 0.7370703575547866}{\scriptsize{ 0.060}} & \cellcolor[rgb]{0.5478662053056518, 0.8232987312572089, 0.7284890426758939}{\scriptsize{ 0.051}} \\
\cellcolor[rgb]{0.1331026528258362, 0.5885428681276432, 0.7550941945405614}{\scriptsize{ 0.165}} & \cellcolor[rgb]{0.33499423298731257, 0.7434371395617071, 0.7570011534025375}{\scriptsize{ 0.083}} &   \cellcolor[rgb]{0.4189004229142639, 0.774563629373318, 0.7448212226066897}{\scriptsize{ 0.068}} &  \cellcolor[rgb]{0.4722952710495963, 0.7943713956170704, 0.7370703575547866}{\scriptsize{ 0.060}} & \cellcolor[rgb]{0.5390080738177624, 0.8198539023452518, 0.7293502499038831}{\scriptsize{ 0.052}} \\
\cellcolor[rgb]{0.1331026528258362, 0.5885428681276432, 0.7550941945405614}{\scriptsize{ 0.164}} & \cellcolor[rgb]{0.34262206843521725, 0.7462668204536717, 0.7558938869665514}{\scriptsize{ 0.082}} & \cellcolor[rgb]{0.39601691657054977, 0.7660745866974241, 0.7481430219146482}{\scriptsize{ 0.072}} &  \cellcolor[rgb]{0.4722952710495963, 0.7943713956170704, 0.7370703575547866}{\scriptsize{ 0.060}} & \cellcolor[rgb]{0.5301499423298732, 0.8164090734332949, 0.7302114571318723}{\scriptsize{ 0.053}} \\
\cellcolor[rgb]{0.11534025374855825, 0.552156862745098, 0.7451903114186851}{\scriptsize{ 0.187}} & \cellcolor[rgb]{0.25871587850826605, 0.7151403306420607, 0.7680738177623991}{\scriptsize{ 0.098}} &  \cellcolor[rgb]{0.3731334102268358, 0.7575855440215302, 0.7514648212226067}{\scriptsize{ 0.076}} & \cellcolor[rgb]{0.43415609381007303, 0.7802229911572472, 0.7426066897347174}{\scriptsize{ 0.065}} &   \cellcolor[rgb]{0.5035755478662054, 0.8060745866974242, 0.73279507881584}{\scriptsize{ 0.055}} \\
\cellcolor[rgb]{0.11964628988850443, 0.508235294117647, 0.7245213379469435}{\scriptsize{ 0.209}} &   \cellcolor[rgb]{0.2968550557477894, 0.729288735101884, 0.7625374855824683}{\scriptsize{ 0.090}} &    \cellcolor[rgb]{0.3578777393310266, 0.751926182237601, 0.753679354094579}{\scriptsize{ 0.079}} &  \cellcolor[rgb]{0.4722952710495963, 0.7943713956170704, 0.7370703575547866}{\scriptsize{ 0.060}} & \cellcolor[rgb]{0.4875509419454056, 0.8000307574009996, 0.7348558246828143}{\scriptsize{ 0.057}} \\
\bottomrule
\end{tabular}


==> fig/lxf_5_rmse1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.14196078431372547, 0.5976470588235294, 0.756078431372549}{\scriptsize{ 0.157}} &  \cellcolor[rgb]{0.2892272202998847, 0.7264590542099193, 0.7636447520184545}{\scriptsize{ 0.093}} &   \cellcolor[rgb]{0.3121107266435986, 0.7349480968858132, 0.760322952710496}{\scriptsize{ 0.088}} &  \cellcolor[rgb]{0.3197385620915033, 0.7377777777777779, 0.7592156862745099}{\scriptsize{ 0.086}} &   \cellcolor[rgb]{0.4799231064975011, 0.797201076509035, 0.7359630911188004}{\scriptsize{ 0.059}} \\
\cellcolor[rgb]{0.1331026528258362, 0.5885428681276432, 0.7550941945405614}{\scriptsize{ 0.165}} &  \cellcolor[rgb]{0.2892272202998847, 0.7264590542099193, 0.7636447520184545}{\scriptsize{ 0.092}} &  \cellcolor[rgb]{0.3273663975394079, 0.7406074586697424, 0.7581084198385236}{\scriptsize{ 0.085}} & \cellcolor[rgb]{0.33499423298731257, 0.7434371395617071, 0.7570011534025375}{\scriptsize{ 0.082}} &  \cellcolor[rgb]{0.4875509419454056, 0.8000307574009996, 0.7348558246828143}{\scriptsize{ 0.058}} \\
\cellcolor[rgb]{0.1331026528258362, 0.5885428681276432, 0.7550941945405614}{\scriptsize{ 0.164}} &   \cellcolor[rgb]{0.2968550557477894, 0.729288735101884, 0.7625374855824683}{\scriptsize{ 0.091}} &  \cellcolor[rgb]{0.3197385620915033, 0.7377777777777779, 0.7592156862745099}{\scriptsize{ 0.086}} & \cellcolor[rgb]{0.34262206843521725, 0.7462668204536717, 0.7558938869665514}{\scriptsize{ 0.081}} &   \cellcolor[rgb]{0.4951787773933103, 0.8028604382929643, 0.733748558246828}{\scriptsize{ 0.057}} \\
\cellcolor[rgb]{0.11534025374855825, 0.552156862745098, 0.7451903114186851}{\scriptsize{ 0.187}} & \cellcolor[rgb]{0.24825836216839675, 0.7068973471741637, 0.7678892733564014}{\scriptsize{ 0.103}} & \cellcolor[rgb]{0.30448289119569394, 0.7321184159938485, 0.7614302191464821}{\scriptsize{ 0.089}} & \cellcolor[rgb]{0.33499423298731257, 0.7434371395617071, 0.7570011534025375}{\scriptsize{ 0.083}} & \cellcolor[rgb]{0.38838908112264514, 0.7632449058054595, 0.7492502883506343}{\scriptsize{ 0.073}} \\
\cellcolor[rgb]{0.11964628988850443, 0.508235294117647, 0.7245213379469435}{\scriptsize{ 0.209}} &  \cellcolor[rgb]{0.26634371395617074, 0.7179700115340254, 0.766966551326413}{\scriptsize{ 0.096}} &   \cellcolor[rgb]{0.2968550557477894, 0.729288735101884, 0.7625374855824683}{\scriptsize{ 0.091}} &  \cellcolor[rgb]{0.4722952710495963, 0.7943713956170704, 0.7370703575547866}{\scriptsize{ 0.060}} &  \cellcolor[rgb]{0.4875509419454056, 0.8000307574009996, 0.7348558246828143}{\scriptsize{ 0.058}} \\
\bottomrule
\end{tabular}


==> fig/t_discr.tex <==
\begin{tabular}{C{3ex}|}

  5 \\
 11 \\
 21 \\
 31 \\
 51 \\

\end{tabular}


==> fig/tn_discr.tex <==
\begin{tabular}{|R{3ex}|}

       \\
       \\
 $N_t$ \\
       \\
       \\

\end{tabular}


==> fig/trm_1_param0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.9078046905036524, 0.32425990003844674, 0.21537870049980778}{\scriptsize{ 0.84}} &   \cellcolor[rgb]{0.9988465974625145, 0.964244521337947, 0.689042675893887}{\scriptsize{ 0.53}} & \cellcolor[rgb]{0.7333333333333333, 0.8865051903114186, 0.4689734717416378}{\scriptsize{ 0.34}} & \cellcolor[rgb]{0.4787389465590157, 0.7756247597078046, 0.3968473663975394}{\scriptsize{ 0.23}} & \cellcolor[rgb]{0.21299500192233758, 0.6501345636293733, 0.34148404459823145}{\scriptsize{ 0.14}} \\
 \cellcolor[rgb]{0.8988850442137639, 0.3054978854286813, 0.20676662821991543}{\scriptsize{ 0.85}} & \cellcolor[rgb]{0.9983852364475202, 0.9499423298731258, 0.6650519031141869}{\scriptsize{ 0.54}} &  \cellcolor[rgb]{0.8039215686274509, 0.916955017301038, 0.5146482122260668}{\scriptsize{ 0.38}} & \cellcolor[rgb]{0.5279507881584006, 0.7971549404075355, 0.4022299115724721}{\scriptsize{ 0.25}} & \cellcolor[rgb]{0.27143406382160706, 0.6785851595540177, 0.35609381007304886}{\scriptsize{ 0.16}} \\
 \cellcolor[rgb]{0.8944252210688197, 0.2961168781237985, 0.20246059207996925}{\scriptsize{ 0.85}} & \cellcolor[rgb]{0.9982314494425221, 0.9451749327181853, 0.6570549788542869}{\scriptsize{ 0.55}} & \cellcolor[rgb]{0.8274509803921568, 0.9271049596309112, 0.5298731257208765}{\scriptsize{ 0.39}} & \cellcolor[rgb]{0.5476355247981544, 0.8057670126874278, 0.4043829296424452}{\scriptsize{ 0.26}} &  \cellcolor[rgb]{0.29480968858131495, 0.6899653979238755, 0.3619377162629758}{\scriptsize{ 0.16}} \\
 \cellcolor[rgb]{0.8944252210688197, 0.2961168781237985, 0.20246059207996925}{\scriptsize{ 0.85}} & \cellcolor[rgb]{0.9982314494425221, 0.9451749327181853, 0.6570549788542869}{\scriptsize{ 0.55}} & \cellcolor[rgb]{0.8274509803921568, 0.9271049596309112, 0.5298731257208765}{\scriptsize{ 0.39}} & \cellcolor[rgb]{0.5574778931180314, 0.8100730488273741, 0.4054594386774318}{\scriptsize{ 0.26}} &  \cellcolor[rgb]{0.29480968858131495, 0.6899653979238755, 0.3619377162629758}{\scriptsize{ 0.17}} \\
 \cellcolor[rgb]{0.8944252210688197, 0.2961168781237985, 0.20246059207996925}{\scriptsize{ 0.85}} &   \cellcolor[rgb]{0.998077662437524, 0.940407535563245, 0.6490580545943868}{\scriptsize{ 0.55}} & \cellcolor[rgb]{0.8352941176470587, 0.9304882737408688, 0.5349480968858131}{\scriptsize{ 0.39}} & \cellcolor[rgb]{0.5574778931180314, 0.8100730488273741, 0.4054594386774318}{\scriptsize{ 0.26}} &  \cellcolor[rgb]{0.29480968858131495, 0.6899653979238755, 0.3619377162629758}{\scriptsize{ 0.17}} \\
\bottomrule
\end{tabular}


==> fig/trm_1_param1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.8498269896193773, 0.20230680507497142, 0.15940023068050763}{\scriptsize{ 0.89}} & \cellcolor[rgb]{0.9925413302575933, 0.7015763168012306, 0.39653979238754344}{\scriptsize{ 0.69}} &  \cellcolor[rgb]{0.944482891195694, 0.9766243752402922, 0.6730488273740869}{\scriptsize{ 0.46}} & \cellcolor[rgb]{0.6263744713571701, 0.8402153018069972, 0.41299500192233757}{\scriptsize{ 0.29}} &   \cellcolor[rgb]{0.04398308342945021, 0.48904267589388695, 0.2579777008842753}{\scriptsize{ 0.05}} \\
  \cellcolor[rgb]{0.8392925797770089, 0.1845444059976932, 0.1528642829680892}{\scriptsize{ 0.90}} &  \cellcolor[rgb]{0.9930026912725874, 0.7246443675509422, 0.4159169550173012}{\scriptsize{ 0.68}} & \cellcolor[rgb]{0.9035755478662053, 0.9594002306805075, 0.6170703575547866}{\scriptsize{ 0.44}} &  \cellcolor[rgb]{0.5279507881584006, 0.7971549404075355, 0.4022299115724721}{\scriptsize{ 0.25}} & \cellcolor[rgb]{0.007996924259900038, 0.42260668973471743, 0.22337562475970782}{\scriptsize{ 0.01}} \\
 \cellcolor[rgb]{0.831603229527105, 0.17716262975778546, 0.15271049596309114}{\scriptsize{ 0.90}} &  \cellcolor[rgb]{0.9931564782775856, 0.732333717800846, 0.42237600922722046}{\scriptsize{ 0.67}} & \cellcolor[rgb]{0.8977316416762784, 0.9569396386005382, 0.6090734332948865}{\scriptsize{ 0.43}} &  \cellcolor[rgb]{0.5181084198385236, 0.7928489042675894, 0.4011534025374856}{\scriptsize{ 0.25}} &                  \cellcolor[rgb]{0.0, 0.40784313725490196, 0.21568627450980393}{\scriptsize{ 0.00}} \\
 \cellcolor[rgb]{0.831603229527105, 0.17716262975778546, 0.15271049596309114}{\scriptsize{ 0.91}} & \cellcolor[rgb]{0.9933102652825837, 0.7400230680507499, 0.42883506343713973}{\scriptsize{ 0.67}} &  \cellcolor[rgb]{0.8918877354863514, 0.954479046520569, 0.6010765090349866}{\scriptsize{ 0.43}} & \cellcolor[rgb]{0.5082660515186467, 0.7885428681276432, 0.40007689350249903}{\scriptsize{ 0.24}} & \cellcolor[rgb]{0.003998462129950019, 0.41522491349480967, 0.21953094963475586}{\scriptsize{ 0.01}} \\
 \cellcolor[rgb]{0.831603229527105, 0.17716262975778546, 0.15271049596309114}{\scriptsize{ 0.91}} & \cellcolor[rgb]{0.9933102652825837, 0.7400230680507499, 0.42883506343713973}{\scriptsize{ 0.67}} & \cellcolor[rgb]{0.8860438292964244, 0.9520184544405997, 0.5930795847750865}{\scriptsize{ 0.42}} &   \cellcolor[rgb]{0.4984236831987696, 0.784236831987697, 0.3990003844675125}{\scriptsize{ 0.24}} & \cellcolor[rgb]{0.011995386389850057, 0.42998846597462514, 0.22722029988465975}{\scriptsize{ 0.01}} \\
\bottomrule
\end{tabular}


==> fig/trm_1_rmse0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.46466743560169166, 0.7915417147251057, 0.7381776239907727}{\scriptsize{ 0.061}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} & \cellcolor[rgb]{0.5567243367935409, 0.8267435601691657, 0.7276278354479047}{\scriptsize{ 0.050}} & \cellcolor[rgb]{0.5655824682814302, 0.8301883890811227, 0.7267666282199154}{\scriptsize{ 0.049}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.045}} \\
 \cellcolor[rgb]{0.4875509419454056, 0.8000307574009996, 0.7348558246828143}{\scriptsize{ 0.057}} & \cellcolor[rgb]{0.6364475201845444, 0.8577470203767782, 0.7198769703960015}{\scriptsize{ 0.043}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.047}} & \cellcolor[rgb]{0.5744405997693195, 0.8336332179930797, 0.7259054209919261}{\scriptsize{ 0.048}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} \\
   \cellcolor[rgb]{0.5035755478662054, 0.8060745866974242, 0.73279507881584}{\scriptsize{ 0.056}} & \cellcolor[rgb]{0.6453056516724337, 0.8611918492887352, 0.7190157631680123}{\scriptsize{ 0.042}} &  \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.047}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.048}} & \cellcolor[rgb]{0.6098731257208766, 0.8474125336409073, 0.7224605920799693}{\scriptsize{ 0.045}} \\
   \cellcolor[rgb]{0.5035755478662054, 0.8060745866974242, 0.73279507881584}{\scriptsize{ 0.056}} &   \cellcolor[rgb]{0.654163783160323, 0.864636678200692, 0.7181545559400231}{\scriptsize{ 0.041}} &  \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.047}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.048}} & \cellcolor[rgb]{0.6098731257208766, 0.8474125336409073, 0.7224605920799693}{\scriptsize{ 0.045}} \\
   \cellcolor[rgb]{0.5035755478662054, 0.8060745866974242, 0.73279507881584}{\scriptsize{ 0.055}} &   \cellcolor[rgb]{0.654163783160323, 0.864636678200692, 0.7181545559400231}{\scriptsize{ 0.041}} &  \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.046}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.048}} & \cellcolor[rgb]{0.6098731257208766, 0.8474125336409073, 0.7224605920799693}{\scriptsize{ 0.045}} \\
\bottomrule
\end{tabular}


==> fig/trm_1_rmse1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.45703960015378703, 0.7887120338331411, 0.7392848904267589}{\scriptsize{ 0.062}} & \cellcolor[rgb]{0.5744405997693195, 0.8336332179930797, 0.7259054209919261}{\scriptsize{ 0.049}} & \cellcolor[rgb]{0.5390080738177624, 0.8198539023452518, 0.7293502499038831}{\scriptsize{ 0.052}} & \cellcolor[rgb]{0.5655824682814302, 0.8301883890811227, 0.7267666282199154}{\scriptsize{ 0.049}} & \cellcolor[rgb]{0.6010149942329873, 0.8439677047289504, 0.7233217993079585}{\scriptsize{ 0.045}} \\
  \cellcolor[rgb]{0.4799231064975011, 0.797201076509035, 0.7359630911188004}{\scriptsize{ 0.059}} & \cellcolor[rgb]{0.6010149942329873, 0.8439677047289504, 0.7233217993079585}{\scriptsize{ 0.046}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.047}} & \cellcolor[rgb]{0.5744405997693195, 0.8336332179930797, 0.7259054209919261}{\scriptsize{ 0.048}} &  \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.046}} \\
 \cellcolor[rgb]{0.4875509419454056, 0.8000307574009996, 0.7348558246828143}{\scriptsize{ 0.057}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} &  \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.047}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.048}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.047}} \\
  \cellcolor[rgb]{0.4951787773933103, 0.8028604382929643, 0.733748558246828}{\scriptsize{ 0.057}} & \cellcolor[rgb]{0.6275893886966551, 0.8543021914648212, 0.7207381776239907}{\scriptsize{ 0.044}} &  \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.047}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.048}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.047}} \\
  \cellcolor[rgb]{0.4951787773933103, 0.8028604382929643, 0.733748558246828}{\scriptsize{ 0.056}} & \cellcolor[rgb]{0.6275893886966551, 0.8543021914648212, 0.7207381776239907}{\scriptsize{ 0.043}} &  \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.047}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.048}} & \cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.047}} \\
\bottomrule
\end{tabular}


==> fig/trm_3_param0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
 \cellcolor[rgb]{0.9922337562475971, 0.6861976163014227, 0.3836216839677049}{\scriptsize{ 0.70}} & \cellcolor[rgb]{0.41968473663975386, 0.7497885428681277, 0.39038831218762016}{\scriptsize{ 0.21}} &  \cellcolor[rgb]{0.15455594002306805, 0.621683967704729, 0.32687427912341405}{\scriptsize{ 0.12}} &  \cellcolor[rgb]{0.0839677047289504, 0.5628604382929643, 0.2964244521337947}{\scriptsize{ 0.09}} & \cellcolor[rgb]{0.0639753940792003, 0.5259515570934256, 0.27720107650903497}{\scriptsize{ 0.06}} \\
 \cellcolor[rgb]{0.9831603229527106, 0.617377931564783, 0.35040369088812007}{\scriptsize{ 0.72}} &   \cellcolor[rgb]{0.43936947327950787, 0.75840061514802, 0.39254133025759325}{\scriptsize{ 0.22}} & \cellcolor[rgb]{0.21299500192233758, 0.6501345636293733, 0.34148404459823145}{\scriptsize{ 0.14}} & \cellcolor[rgb]{0.09596309111880046, 0.5850057670126874, 0.3079584775086505}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.0639753940792003, 0.5259515570934256, 0.27720107650903497}{\scriptsize{ 0.07}} \\
\cellcolor[rgb]{0.9790080738177624, 0.5873894655901578, 0.33656286043829303}{\scriptsize{ 0.74}} &  \cellcolor[rgb]{0.4492118415993849, 0.7627066512879662, 0.39361783929257976}{\scriptsize{ 0.22}} &  \cellcolor[rgb]{0.2363706266820453, 0.6615148019992311, 0.34732795078815837}{\scriptsize{ 0.14}} & \cellcolor[rgb]{0.09996155324875047, 0.5923875432525951, 0.3118031526336025}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.0639753940792003, 0.5259515570934256, 0.27720107650903497}{\scriptsize{ 0.07}} \\
 \cellcolor[rgb]{0.9776239907727797, 0.5773933102652827, 0.3319492502883507}{\scriptsize{ 0.74}} &  \cellcolor[rgb]{0.4492118415993849, 0.7627066512879662, 0.39361783929257976}{\scriptsize{ 0.22}} &  \cellcolor[rgb]{0.2363706266820453, 0.6615148019992311, 0.34732795078815837}{\scriptsize{ 0.15}} & \cellcolor[rgb]{0.09996155324875047, 0.5923875432525951, 0.3118031526336025}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.0639753940792003, 0.5259515570934256, 0.27720107650903497}{\scriptsize{ 0.07}} \\
 \cellcolor[rgb]{0.9776239907727797, 0.5773933102652827, 0.3319492502883507}{\scriptsize{ 0.74}} &  \cellcolor[rgb]{0.4492118415993849, 0.7627066512879662, 0.39361783929257976}{\scriptsize{ 0.22}} &  \cellcolor[rgb]{0.2363706266820453, 0.6615148019992311, 0.34732795078815837}{\scriptsize{ 0.15}} & \cellcolor[rgb]{0.09996155324875047, 0.5923875432525951, 0.3118031526336025}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.0639753940792003, 0.5259515570934256, 0.27720107650903497}{\scriptsize{ 0.07}} \\
\bottomrule
\end{tabular}


==> fig/trm_3_param1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.8721261053440984, 0.24921184159938484, 0.18093041138023838}{\scriptsize{ 0.87}} & \cellcolor[rgb]{0.7490196078431371, 0.8932718185313341, 0.47912341407151093}{\scriptsize{ 0.35}} & \cellcolor[rgb]{0.011995386389850057, 0.42998846597462514, 0.22722029988465975}{\scriptsize{ 0.01}} & \cellcolor[rgb]{0.3064975009611688, 0.6956555171088044, 0.36485966935793923}{\scriptsize{ 0.17}} &   \cellcolor[rgb]{0.5870049980776624, 0.8229911572472126, 0.4086889657823914}{\scriptsize{ 0.27}} \\
\cellcolor[rgb]{0.8587466359092657, 0.22106881968473663, 0.16801230296039987}{\scriptsize{ 0.89}} & \cellcolor[rgb]{0.7176470588235293, 0.8797385620915033, 0.45882352941176463}{\scriptsize{ 0.34}} &  \cellcolor[rgb]{0.03198769703960015, 0.46689734717416376, 0.24644367550941945}{\scriptsize{ 0.03}} &                \cellcolor[rgb]{0.4, 0.7411764705882353, 0.38823529411764707}{\scriptsize{ 0.20}} &   \cellcolor[rgb]{0.4295271049596309, 0.7540945790080739, 0.3914648212226067}{\scriptsize{ 0.21}} \\
  \cellcolor[rgb]{0.8542868127643214, 0.2116878123798539, 0.1637062668204537}{\scriptsize{ 0.89}} & \cellcolor[rgb]{0.7019607843137254, 0.8729719338715878, 0.44867358708189153}{\scriptsize{ 0.32}} &  \cellcolor[rgb]{0.03198769703960015, 0.46689734717416376, 0.24644367550941945}{\scriptsize{ 0.03}} & \cellcolor[rgb]{0.37662437524029213, 0.7297962322183775, 0.3823913879277201}{\scriptsize{ 0.19}} &                 \cellcolor[rgb]{0.4, 0.7411764705882353, 0.38823529411764707}{\scriptsize{ 0.20}} \\
 \cellcolor[rgb]{0.6460592079969241, 0.8488273740868896, 0.41514801999231066}{\scriptsize{ 0.30}} &  \cellcolor[rgb]{0.6862745098039215, 0.8662053056516724, 0.4385236447520184}{\scriptsize{ 0.32}} &   \cellcolor[rgb]{0.035986159169550176, 0.4742791234140715, 0.2502883506343714}{\scriptsize{ 0.04}} &  \cellcolor[rgb]{0.3883121876201462, 0.7354863514033064, 0.3853133410226836}{\scriptsize{ 0.20}} &                 \cellcolor[rgb]{0.4, 0.7411764705882353, 0.38823529411764707}{\scriptsize{ 0.20}} \\
\cellcolor[rgb]{0.8498269896193773, 0.20230680507497142, 0.15940023068050763}{\scriptsize{ 0.89}} &  \cellcolor[rgb]{0.6862745098039215, 0.8662053056516724, 0.4385236447520184}{\scriptsize{ 0.32}} &   \cellcolor[rgb]{0.04398308342945021, 0.48904267589388695, 0.2579777008842753}{\scriptsize{ 0.04}} & \cellcolor[rgb]{0.40984236831987697, 0.7454825067281815, 0.3893118031526336}{\scriptsize{ 0.20}} & \cellcolor[rgb]{0.41968473663975386, 0.7497885428681277, 0.39038831218762016}{\scriptsize{ 0.21}} \\
\bottomrule
\end{tabular}


==> fig/trm_3_rmse0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.4875509419454056, 0.8000307574009996, 0.7348558246828143}{\scriptsize{ 0.058}} &  \cellcolor[rgb]{0.8587004998077663, 0.944636678200692, 0.6997001153402538}{\scriptsize{ 0.023}} & \cellcolor[rgb]{0.7838985005767013, 0.9151095732410611, 0.7056055363321799}{\scriptsize{ 0.032}} & \cellcolor[rgb]{0.7693194925028836, 0.9094194540561322, 0.7069588619761631}{\scriptsize{ 0.033}} &  \cellcolor[rgb]{0.797923875432526, 0.9206459054209919, 0.7044982698961938}{\scriptsize{ 0.030}} \\
 \cellcolor[rgb]{0.5124336793540947, 0.809519415609381, 0.7319338715878507}{\scriptsize{ 0.055}} & \cellcolor[rgb]{0.8446751249519415, 0.9391003460207612, 0.7008073817762399}{\scriptsize{ 0.025}} &  \cellcolor[rgb]{0.7885736255286429, 0.916955017301038, 0.7052364475201846}{\scriptsize{ 0.031}} & \cellcolor[rgb]{0.7693194925028836, 0.9094194540561322, 0.7069588619761631}{\scriptsize{ 0.033}} & \cellcolor[rgb]{0.8119492502883506, 0.9261822376009227, 0.7033910034602077}{\scriptsize{ 0.028}} \\
  \cellcolor[rgb]{0.521291810841984, 0.812964244521338, 0.7310726643598615}{\scriptsize{ 0.054}} & \cellcolor[rgb]{0.8540253748558247, 0.9427912341407151, 0.7000692041522492}{\scriptsize{ 0.024}} & \cellcolor[rgb]{0.7838985005767013, 0.9151095732410611, 0.7056055363321799}{\scriptsize{ 0.031}} & \cellcolor[rgb]{0.7693194925028836, 0.9094194540561322, 0.7069588619761631}{\scriptsize{ 0.033}} &  \cellcolor[rgb]{0.8072741253364091, 0.9243367935409458, 0.703760092272203}{\scriptsize{ 0.029}} \\
  \cellcolor[rgb]{0.521291810841984, 0.812964244521338, 0.7310726643598615}{\scriptsize{ 0.053}} & \cellcolor[rgb]{0.8540253748558247, 0.9427912341407151, 0.7000692041522492}{\scriptsize{ 0.024}} & \cellcolor[rgb]{0.7838985005767013, 0.9151095732410611, 0.7056055363321799}{\scriptsize{ 0.032}} & \cellcolor[rgb]{0.7604613610149944, 0.9059746251441754, 0.7078200692041523}{\scriptsize{ 0.033}} & \cellcolor[rgb]{0.8025990003844675, 0.9224913494809688, 0.7041291810841984}{\scriptsize{ 0.029}} \\
\cellcolor[rgb]{0.5301499423298732, 0.8164090734332949, 0.7302114571318723}{\scriptsize{ 0.053}} & \cellcolor[rgb]{0.8540253748558247, 0.9427912341407151, 0.7000692041522492}{\scriptsize{ 0.024}} & \cellcolor[rgb]{0.7838985005767013, 0.9151095732410611, 0.7056055363321799}{\scriptsize{ 0.031}} & \cellcolor[rgb]{0.7693194925028836, 0.9094194540561322, 0.7069588619761631}{\scriptsize{ 0.033}} & \cellcolor[rgb]{0.8025990003844675, 0.9224913494809688, 0.7041291810841984}{\scriptsize{ 0.029}} \\
\bottomrule
\end{tabular}


==> fig/trm_3_rmse1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.46466743560169166, 0.7915417147251057, 0.7381776239907727}{\scriptsize{ 0.061}} & \cellcolor[rgb]{0.8259746251441753, 0.9317185697808535, 0.7022837370242214}{\scriptsize{ 0.027}} & \cellcolor[rgb]{0.7427450980392157, 0.8990849673202614, 0.7095424836601307}{\scriptsize{ 0.034}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} & \cellcolor[rgb]{0.5301499423298732, 0.8164090734332949, 0.7302114571318723}{\scriptsize{ 0.053}} \\
 \cellcolor[rgb]{0.4875509419454056, 0.8000307574009996, 0.7348558246828143}{\scriptsize{ 0.058}} & \cellcolor[rgb]{0.8259746251441753, 0.9317185697808535, 0.7022837370242214}{\scriptsize{ 0.027}} & \cellcolor[rgb]{0.7427450980392157, 0.8990849673202614, 0.7095424836601307}{\scriptsize{ 0.034}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} \\
  \cellcolor[rgb]{0.4951787773933103, 0.8028604382929643, 0.733748558246828}{\scriptsize{ 0.057}} & \cellcolor[rgb]{0.8353248750480584, 0.9354094579008073, 0.7015455594002307}{\scriptsize{ 0.026}} & \cellcolor[rgb]{0.7338869665513265, 0.8956401384083045, 0.7104036908881199}{\scriptsize{ 0.035}} & \cellcolor[rgb]{0.6275893886966551, 0.8543021914648212, 0.7207381776239907}{\scriptsize{ 0.044}} & \cellcolor[rgb]{0.6364475201845444, 0.8577470203767782, 0.7198769703960015}{\scriptsize{ 0.043}} \\
\cellcolor[rgb]{0.44941176470588234, 0.7858823529411765, 0.7403921568627451}{\scriptsize{ 0.063}} &               \cellcolor[rgb]{0.84, 0.9372549019607843, 0.7011764705882353}{\scriptsize{ 0.025}} & \cellcolor[rgb]{0.7338869665513265, 0.8956401384083045, 0.7104036908881199}{\scriptsize{ 0.035}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} & \cellcolor[rgb]{0.6364475201845444, 0.8577470203767782, 0.7198769703960015}{\scriptsize{ 0.043}} \\
   \cellcolor[rgb]{0.5035755478662054, 0.8060745866974242, 0.73279507881584}{\scriptsize{ 0.056}} &               \cellcolor[rgb]{0.84, 0.9372549019607843, 0.7011764705882353}{\scriptsize{ 0.025}} & \cellcolor[rgb]{0.7250288350634372, 0.8921953094963475, 0.7112648981161093}{\scriptsize{ 0.035}} &  \cellcolor[rgb]{0.618731257208766, 0.8508573625528644, 0.7215993848519799}{\scriptsize{ 0.044}} & \cellcolor[rgb]{0.6275893886966551, 0.8543021914648212, 0.7207381776239907}{\scriptsize{ 0.043}} \\
\bottomrule
\end{tabular}


==> fig/trm_5_param0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
 \cellcolor[rgb]{0.944482891195694, 0.9766243752402922, 0.6730488273740869}{\scriptsize{ 0.46}} &   \cellcolor[rgb]{0.1896193771626297, 0.6387543252595156, 0.3356401384083045}{\scriptsize{ 0.13}} & \cellcolor[rgb]{0.08796616685890042, 0.5702422145328719, 0.30026912725874666}{\scriptsize{ 0.09}} & \cellcolor[rgb]{0.05997693194925029, 0.5185697808535179, 0.27335640138408307}{\scriptsize{ 0.06}} & \cellcolor[rgb]{0.03998462129950019, 0.48166089965397924, 0.25413302575932334}{\scriptsize{ 0.04}} \\
\cellcolor[rgb]{0.9737024221453288, 0.9889273356401385, 0.7130334486735871}{\scriptsize{ 0.48}} &   \cellcolor[rgb]{0.20130718954248367, 0.6444444444444445, 0.338562091503268}{\scriptsize{ 0.14}} &  \cellcolor[rgb]{0.09596309111880046, 0.5850057670126874, 0.3079584775086505}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.06797385620915032, 0.5333333333333333, 0.28104575163398693}{\scriptsize{ 0.07}} & \cellcolor[rgb]{0.03998462129950019, 0.48166089965397924, 0.25413302575932334}{\scriptsize{ 0.04}} \\
\cellcolor[rgb]{0.9853902345251826, 0.9938485198000769, 0.7290272971933871}{\scriptsize{ 0.49}} & \cellcolor[rgb]{0.21299500192233758, 0.6501345636293733, 0.34148404459823145}{\scriptsize{ 0.14}} & \cellcolor[rgb]{0.10780469050365243, 0.5989234909650134, 0.31518646674356016}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.06797385620915032, 0.5333333333333333, 0.28104575163398693}{\scriptsize{ 0.07}} & \cellcolor[rgb]{0.03998462129950019, 0.48166089965397924, 0.25413302575932334}{\scriptsize{ 0.04}} \\
\cellcolor[rgb]{0.9912341407151095, 0.9963091118800461, 0.7370242214532872}{\scriptsize{ 0.49}} & \cellcolor[rgb]{0.21299500192233758, 0.6501345636293733, 0.34148404459823145}{\scriptsize{ 0.14}} & \cellcolor[rgb]{0.10780469050365243, 0.5989234909650134, 0.31518646674356016}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.06797385620915032, 0.5333333333333333, 0.28104575163398693}{\scriptsize{ 0.07}} & \cellcolor[rgb]{0.03998462129950019, 0.48166089965397924, 0.25413302575932334}{\scriptsize{ 0.04}} \\
\cellcolor[rgb]{0.9912341407151095, 0.9963091118800461, 0.7370242214532872}{\scriptsize{ 0.50}} & \cellcolor[rgb]{0.21299500192233758, 0.6501345636293733, 0.34148404459823145}{\scriptsize{ 0.14}} & \cellcolor[rgb]{0.10780469050365243, 0.5989234909650134, 0.31518646674356016}{\scriptsize{ 0.10}} & \cellcolor[rgb]{0.06797385620915032, 0.5333333333333333, 0.28104575163398693}{\scriptsize{ 0.07}} & \cellcolor[rgb]{0.03998462129950019, 0.48166089965397924, 0.25413302575932334}{\scriptsize{ 0.04}} \\
\bottomrule
\end{tabular}


==> fig/trm_5_param1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
   \cellcolor[rgb]{0.9033448673587082, 0.314878892733564, 0.2110726643598616}{\scriptsize{ 0.85}} &  \cellcolor[rgb]{0.14286812764321416, 0.6159938485198001, 0.3239523260284506}{\scriptsize{ 0.12}} &   \cellcolor[rgb]{0.32987312572087657, 0.707035755478662, 0.3707035755478662}{\scriptsize{ 0.18}} & \cellcolor[rgb]{0.5968473663975393, 0.8272971933871587, 0.40976547481737796}{\scriptsize{ 0.28}} &  \cellcolor[rgb]{0.14286812764321416, 0.6159938485198001, 0.3239523260284506}{\scriptsize{ 0.12}} \\
 \cellcolor[rgb]{0.8810457516339869, 0.2679738562091503, 0.18954248366013074}{\scriptsize{ 0.86}} &  \cellcolor[rgb]{0.09596309111880046, 0.5850057670126874, 0.3079584775086505}{\scriptsize{ 0.10}} &   \cellcolor[rgb]{0.3415609381007305, 0.7127258746635909, 0.3736255286428297}{\scriptsize{ 0.18}} &  \cellcolor[rgb]{0.5377931564782775, 0.8014609765474817, 0.4033064206074587}{\scriptsize{ 0.25}} &   \cellcolor[rgb]{0.0839677047289504, 0.5628604382929643, 0.2964244521337947}{\scriptsize{ 0.08}} \\
  \cellcolor[rgb]{0.8431372549019608, 0.9338715878508266, 0.5400230680507496}{\scriptsize{ 0.40}} & \cellcolor[rgb]{0.07996924259900039, 0.5554786620530565, 0.29257977700884275}{\scriptsize{ 0.08}} & \cellcolor[rgb]{0.31818531334102274, 0.7013456362937331, 0.36778162245290275}{\scriptsize{ 0.18}} &  \cellcolor[rgb]{0.43936947327950787, 0.75840061514802, 0.39254133025759325}{\scriptsize{ 0.22}} &  \cellcolor[rgb]{0.07197231833910035, 0.5407151095732411, 0.2848904267589389}{\scriptsize{ 0.07}} \\
                \cellcolor[rgb]{0.6470588235294118, 0.0, 0.14901960784313725}{\scriptsize{ 1.00}} & \cellcolor[rgb]{0.07597078046905037, 0.5480968858131487, 0.28873510188389084}{\scriptsize{ 0.08}} &   \cellcolor[rgb]{0.3415609381007305, 0.7127258746635909, 0.3736255286428297}{\scriptsize{ 0.18}} & \cellcolor[rgb]{0.4492118415993849, 0.7627066512879662, 0.39361783929257976}{\scriptsize{ 0.22}} &  \cellcolor[rgb]{0.07197231833910035, 0.5407151095732411, 0.2848904267589389}{\scriptsize{ 0.07}} \\
\cellcolor[rgb]{0.8721261053440984, 0.24921184159938484, 0.18093041138023838}{\scriptsize{ 0.87}} &  \cellcolor[rgb]{0.07197231833910035, 0.5407151095732411, 0.2848904267589389}{\scriptsize{ 0.07}} &  \cellcolor[rgb]{0.35324875048058446, 0.7184159938485198, 0.3765474817377932}{\scriptsize{ 0.19}} & \cellcolor[rgb]{0.4492118415993849, 0.7627066512879662, 0.39361783929257976}{\scriptsize{ 0.22}} & \cellcolor[rgb]{0.07597078046905037, 0.5480968858131487, 0.28873510188389084}{\scriptsize{ 0.08}} \\
\bottomrule
\end{tabular}


==> fig/trm_5_rmse0.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.5655824682814302, 0.8301883890811227, 0.7267666282199154}{\scriptsize{ 0.050}} & \cellcolor[rgb]{0.9379930795847751, 0.9758861976163014, 0.7131872356785851}{\scriptsize{ 0.017}} & \cellcolor[rgb]{0.8353248750480584, 0.9354094579008073, 0.7015455594002307}{\scriptsize{ 0.025}} &   \cellcolor[rgb]{0.830649750096117, 0.9335640138408304, 0.701914648212226}{\scriptsize{ 0.026}} &  \cellcolor[rgb]{0.872725874663591, 0.9501730103806229, 0.6985928489042675}{\scriptsize{ 0.022}} \\
\cellcolor[rgb]{0.5744405997693195, 0.8336332179930797, 0.7259054209919261}{\scriptsize{ 0.048}} & \cellcolor[rgb]{0.9194771241830065, 0.9686274509803922, 0.6949019607843137}{\scriptsize{ 0.019}} &               \cellcolor[rgb]{0.84, 0.9372549019607843, 0.7011764705882353}{\scriptsize{ 0.025}} &   \cellcolor[rgb]{0.830649750096117, 0.9335640138408304, 0.701914648212226}{\scriptsize{ 0.026}} &  \cellcolor[rgb]{0.8914263744713572, 0.9575547866205305, 0.697116493656286}{\scriptsize{ 0.021}} \\
\cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.047}} &  \cellcolor[rgb]{0.9241522491349482, 0.970472895040369, 0.6945328719723183}{\scriptsize{ 0.018}} &   \cellcolor[rgb]{0.830649750096117, 0.9335640138408304, 0.701914648212226}{\scriptsize{ 0.026}} &   \cellcolor[rgb]{0.830649750096117, 0.9335640138408304, 0.701914648212226}{\scriptsize{ 0.026}} & \cellcolor[rgb]{0.8820761245674741, 0.9538638985005767, 0.6978546712802768}{\scriptsize{ 0.021}} \\
\cellcolor[rgb]{0.5832987312572088, 0.8370780469050365, 0.7250442137639369}{\scriptsize{ 0.047}} &  \cellcolor[rgb]{0.9241522491349482, 0.970472895040369, 0.6945328719723183}{\scriptsize{ 0.018}} &   \cellcolor[rgb]{0.830649750096117, 0.9335640138408304, 0.701914648212226}{\scriptsize{ 0.026}} & \cellcolor[rgb]{0.8259746251441753, 0.9317185697808535, 0.7022837370242214}{\scriptsize{ 0.027}} & \cellcolor[rgb]{0.8820761245674741, 0.9538638985005767, 0.6978546712802768}{\scriptsize{ 0.022}} \\
 \cellcolor[rgb]{0.592156862745098, 0.8405228758169935, 0.7241830065359477}{\scriptsize{ 0.047}} &  \cellcolor[rgb]{0.9241522491349482, 0.970472895040369, 0.6945328719723183}{\scriptsize{ 0.018}} &   \cellcolor[rgb]{0.830649750096117, 0.9335640138408304, 0.701914648212226}{\scriptsize{ 0.026}} & \cellcolor[rgb]{0.8259746251441753, 0.9317185697808535, 0.7022837370242214}{\scriptsize{ 0.026}} & \cellcolor[rgb]{0.8820761245674741, 0.9538638985005767, 0.6978546712802768}{\scriptsize{ 0.022}} \\
\bottomrule
\end{tabular}


==> fig/trm_5_rmse1.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
\cellcolor[rgb]{0.4722952710495963, 0.7943713956170704, 0.7370703575547866}{\scriptsize{ 0.060}} & \cellcolor[rgb]{0.9379930795847751, 0.9758861976163014, 0.7131872356785851}{\scriptsize{ 0.017}} & \cellcolor[rgb]{0.6895963091118802, 0.8784159938485199, 0.7147097270280661}{\scriptsize{ 0.038}} & \cellcolor[rgb]{0.5567243367935409, 0.8267435601691657, 0.7276278354479047}{\scriptsize{ 0.050}} & \cellcolor[rgb]{0.7427450980392157, 0.8990849673202614, 0.7095424836601307}{\scriptsize{ 0.034}} \\
 \cellcolor[rgb]{0.4951787773933103, 0.8028604382929643, 0.733748558246828}{\scriptsize{ 0.057}} &  \cellcolor[rgb]{0.914801999231065, 0.9667820069204152, 0.6952710495963091}{\scriptsize{ 0.019}} & \cellcolor[rgb]{0.7073125720876586, 0.8853056516724337, 0.7129873125720877}{\scriptsize{ 0.037}} & \cellcolor[rgb]{0.6098731257208766, 0.8474125336409073, 0.7224605920799693}{\scriptsize{ 0.045}} & \cellcolor[rgb]{0.8166243752402922, 0.9280276816608997, 0.7030219146482123}{\scriptsize{ 0.028}} \\
\cellcolor[rgb]{0.5744405997693195, 0.8336332179930797, 0.7259054209919261}{\scriptsize{ 0.048}} &  \cellcolor[rgb]{0.914801999231065, 0.9667820069204152, 0.6952710495963091}{\scriptsize{ 0.019}} & \cellcolor[rgb]{0.7161707035755479, 0.8887504805843907, 0.7121261053440985}{\scriptsize{ 0.037}} &   \cellcolor[rgb]{0.654163783160323, 0.864636678200692, 0.7181545559400231}{\scriptsize{ 0.041}} & \cellcolor[rgb]{0.8259746251441753, 0.9317185697808535, 0.7022837370242214}{\scriptsize{ 0.027}} \\
\cellcolor[rgb]{0.4265282583621684, 0.7773933102652826, 0.7437139561707036}{\scriptsize{ 0.067}} &  \cellcolor[rgb]{0.914801999231065, 0.9667820069204152, 0.6952710495963091}{\scriptsize{ 0.019}} & \cellcolor[rgb]{0.7073125720876586, 0.8853056516724337, 0.7129873125720877}{\scriptsize{ 0.037}} &   \cellcolor[rgb]{0.654163783160323, 0.864636678200692, 0.7181545559400231}{\scriptsize{ 0.041}} & \cellcolor[rgb]{0.8212995001922337, 0.9298731257208765, 0.7026528258362169}{\scriptsize{ 0.027}} \\
  \cellcolor[rgb]{0.5035755478662054, 0.8060745866974242, 0.73279507881584}{\scriptsize{ 0.055}} &  \cellcolor[rgb]{0.914801999231065, 0.9667820069204152, 0.6952710495963091}{\scriptsize{ 0.019}} & \cellcolor[rgb]{0.7073125720876586, 0.8853056516724337, 0.7129873125720877}{\scriptsize{ 0.037}} &  \cellcolor[rgb]{0.6630219146482123, 0.868081507112649, 0.7172933487120339}{\scriptsize{ 0.041}} & \cellcolor[rgb]{0.8212995001922337, 0.9298731257208765, 0.7026528258362169}{\scriptsize{ 0.027}} \\
\bottomrule
\end{tabular}


==> fig/x_discr.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}

 5 &  11 &  21 &  31 &  51 \\
\bottomrule
\end{tabular}


==> fig/xn_discr.tex <==
\begin{tabular}{C{5ex}C{5ex}C{5ex}C{5ex}C{5ex}}
\toprule
  &   &  $N_x$ &   &   \\
\bottomrule
\end{tabular}

